Bit-pragmatic Deep Neural Network Computing

We quantify a source of ineffectual computations when processing the multiplications of the convolutional layers in Deep Neural Networks (DNNs) and propose Pragmatic (PRA), an architecture that exploits it improving performance and energy efficiency. The source of these ineffectual computations is best understood in the context of conventional multipliers which generate internally multiple terms, that is, products of the multiplicand and powers of two, which added together produce the final product [1]. At runtime, many of these terms are zero as they are generated when the multiplicand is combined with the zero-bits of the multiplicator. While conventional bit-parallel multipliers calculate all terms in parallel to reduce individual product latency, PRA calculates only the non-zero terms using a) on-the-fly conversion of the multiplicator representation into an explicit list of powers of two, and b) hybrid bit-parallel multplicand/bit-serial multiplicator processing units. PRA exploits two sources of ineffectual computations: 1) the aforementioned zero product terms which are the result of the lack of explicitness in the multiplicator representation, and 2) the excess in the representation precision used for both multiplicants and multiplicators, e.g., [2]. Measurements demonstrate that for the convolutional layers, a straightforward variant of PRA improves performance by 2.6x over the DaDiaNao (DaDN) accelerator [3] and by 1.4x over STR [4]. Similarly, PRA improves energy efficiency by 28% and 10% on average compared to DaDN and STR. An improved cross lane synchronication scheme boosts performance improvements to 3.1x over DaDN. Finally, Pragmatic benefits persist even with an 8-bit quantized representation [5].

==> sections/convolutions.tex <==


\begin{figure*}[h]
\centering
\begin{subfigure}[b]{0.40\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/dadiannao-overview}
\caption{}
\label{fig:dadiannao-overview}
\end{subfigure}
\begin{subfigure}[b]{0.5\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/stripes-overview}
\caption{}
\label{fig:stripes-overview}
\end{subfigure}
\caption{a) DaDianNao Tile. b) Stripes Tile. 
}
\end{figure*}

\section{Background}
\label{sec:background}
This work presents \STRL as a modification of the state-of-the-art \BASE accelerator. Accordingly, this section provides the necessary background information: Section~\ref{sec:convolution} reviews the operation of convolutional layers, and Section~\ref{sec:baseline} reviews the baseline accelerator design and how it implements convolutional layers.

\subsection{Convolutional Layer Computation} 
\label{sec:convolution}

\newcommand{\BBj}[1]{ { \mathbb{#1} } }

The input to a convolutional layer is a 3D array. The layer applies $N$ 3D filters in a sliding window fashion using a constant stride $S$ to produce an output 3D array. 
The  input array contains $N_x\times N_y \times I$ real numbers, or \textit{neurons}. The layer applies $N$ filters, each containing $F_x \times F_y \times I$ real numbers, or \textit{synapses}. The layer outputs a $O_x \times O_y \times N$ neuron array (its depth equals the filter count). The neuron arrays can be thought of comprising several \textit{features}, that is 2D arrays stacked along the $i$ dimension, each corresponding to an output feature. The output has $N$ features, each produced by a different filter. Applying the filter identifies where in the input each feature appears. To calculate an output neuron, one filter is applied over a \textit{window}, a sub-array of the input neuron array that has the same dimensions as the filters $F_x \times F_y \times I$. Let $n(x,y,i)$ and $o(x,y,i)$ be respectively input and output neurons, and $s^f(x,y,i)$ be synapses of filter ${f}$.  
The output neuron at position $(\BBj{k},\BBj{l},\BBj{f})$ is calculated as in:

\begin{gather*}
\small
\underbrace{o(\BBj{k},\BBj{l},\BBj{f})}_{\substack{output\\ neuron}} = 
\underbrace{
\sum_{y=0}^{F_y-1} 
\sum_{x=0}^{F_x-1} 
\sum_{i=0}^{I-1} 
\underbrace{s^{\BBj{f}}(y,x,i)}_{synapse} \times 
\underbrace{n(y+\BBj{l} \times S, x+\BBj{k} \times S,i)}_{input\ neuron}
}_{window}
\label{eq:convolution}
\end{gather*}



There is one output neuron per window and filter. The filters are applied repeatedly over different windows moving along the X and Y dimensions using a constant stride $S$ to produce all the output neurons. Accordingly, the output neuron array dimensions are $O_x=(I_x-F_x)/S+1$, $O_y=(I_y-F_y)/S+1$, and $O_i = N$. 

In the rest of this paper, the term \textit{brick} is used to refer to a set of continuous along the $i$ dimension elements of a 3D neuron or synapse array, e.g., $n(x,y,i)...n(x,y,i+15)$. Bricks will be denoted by their origin element with a $B$ subscript, e.g., $n_B(x,y,i)$.
%Figure~\ref{fig:convolution} shows an example with a $3x3x2$ input neuron array, a single $2x2x2$ filter and unit stride producing an output neuron array of $2x2x1$. 

%When an input neuron is zero the corresponding multiplication and addition can be eliminated without altering the output value. These operations consume energy and time.





==> sections/stripes.tex <==

%\section{Stripes: a Bit-Serial Deep Neural Networks Computing Accelerator}
%\label{sec:stripes}
%This section first introduces the baseline system, the state-of-the-art DaDianNao accelerator~\cite{DaDiannao}. Second, we present the \STRL accelerator, where the corresponding computing time of a particular layer is directly proportional to the required numerical precision representation of such layer.

\subsection{Baseline System}
\label{sec:baseline}
% \PJ{Lets use the following terminology:
% Brick: 16 consecutive neurons e.g. n(x,y,0..15). In the baseline these are processed in parallel.
% Slice: partition of the input data e.g. n(*,*,0..15) containing all the bricks at the same depth. Think of slicing as creating bricks from depthwise(in i) columns of data)
% Chunk: 16 bricks that are processed in parallel in \STR
% }
% \fixme{may be rewrite this so that is not identical to ISCA. DO we need to talk about synapse sublanes here?}

\newcommand{\tile}{tile\xspace}
\newcommand{\tiles}{tiles\xspace}
\newcommand{\nfu}{unit\xspace}
\newcommand{\nfus}{units\xspace}


We demonstrate \STR as an extension over the \textit{DaDianNao} state-of-the-art accelerator proposed by Chen \textit{et al.}~\cite{DaDiannao}. Figure~\ref{fig:dadiannao-overview} shows a \BASE \tile. Each \BASE chip comprises 16 such \tiles. 
Each \tile has a synapse buffer (SB) which provides 256 synapses per cycle one per synapse sub-lane. 
The \tile also has an input neuron buffer (NBin) which provides 16 neurons per cycle one per neuron lane, and an neuron output buffer (NBout) which can accept 16 output neurons per cycle. 
The computational logic is called the \textit{Neural Functional Unit (NFU)}, or \textit{\nfu}.
Every cycle, each NFU produces a brick $o_B(q,w,f)$ of partial output neurons.
%16 consecutive along the $i$ dimension partial output neurons, or a partial output neuron \textit{brick}, i.e., $o_B(q,w,f)$
%$o_B(q,w,f)...o(q,w,f+15)$(for clarity, bricks will be denoted by their first element alone and a $B$ subscript, e.g., $o_B(o,w,f)$).  
The NFU does so by processing one input neuron brick $n_B(x,y,i)$ and 16 synapse bricks one from each of 16 filters: $s^f_B(k,l,i)$ through $s^{f+15}_B(k,l,i)$. 
%The NFU does so by processing one input neuron brick $n(x,y,i) ... n(x,y,i+15)$ and 16 synapse bricks one from each of 16 filters: $s^f(k,l,i) ... s^f(k,l,i+15)$ through $s^{f+15}(k,l,i) ... s^{f+15}(k,l,i+15)$. 
For this purpose, the NFU has 16 neuron lanes and 16 filter lanes each with 16 synapse lanes for a total of 256 synapse-lanes. 
Each neuron lane is connected to 16 synapse sub-lanes, one from each of the 16 filter lanes. 
A synapse lane multiplies its synapse with an input neuron and the 16 products from all synapse lanes of a filter are reduced into a partial sum. 
In all, the filter lanes produce each a partial sum per cycle, for a total 16 output neurons per unit. We refer to the logic associated to the production of one output neuron as an \textit{inner product unit (IP)}. 
Once a full window is processed the 16 resulting sums are fed though a non-linear activation funciton, $f$, to produce 16 output neurons.  
The multiplications and reductions needed per cycle are implemented as 256 multipliers one per synapse sub-lane and sixteen 17-input adder trees one per output neuron (16 products plus the partial sum from NBout). 

\BASE's main goal was minimizing off-chip bandwidth while maximizing on-chip compute utilization. To avoid fetching synapses from off-chip the SB is a 32MB eDRAM distributed in 2MB chunks, one per NFU allowing it to store all synapses for the layer(s) being processed for best of class networks. Overall, a \BASE node can process up to 256 filters in parallel, 16 per unit. All inter-layer neuron outputs except for the initial input and final output are stored in shared, 4MB central eDRAM, or \textit{Neuron Memory} (NM). Off-chip accesses are needed only for reading the input image, the synapses once per layer, and for writing the final output.

Processing starts by reading from external memory the first layer's filter synapses, and the input image. The synapses are distributed over  SBs and the input is stored into NM. Each cycle an input neuron brick, $n_B(x,y,i)$, 
%$n(x,y,i)...n(x,y,i+15)$,
is broadcast to all units. The layer's output neurons are stored through NBout to NM and then fed back through the NBins when processing the next layer. Loading the next set of synapses from external memory can be overlapped with the processing of the current layer as necessary.  


\section{Stripes} 
\label{sec:design}
%This section presents the \STRL design. The description initially focuses on convolutional layers alone, however, like \BASE, \STR can implement all layer types as Section~\ref{sec:fclayer} explains.

%Figure~\ref{fig:stripes-overview} shows an \STR \tile that 1)~offers the same computation throughput as a \BASE \tile, and 2)~needs $p$ cycles to process input neurons represented in $p$ bits.  
This section describes the \STRL design. 
Figure~\ref{fig:systems-overview} shows an overview of the complete \BASE and \STR systems. Both systems use the same NM reading and writing interconnect structures and store neurons in 16-bit containers in NM regardless of the precision used. \STR introduces a \textit{Dispatcher} unit to read neurons from NM using the existing bit-parallel interface while feeding them to the NFUs bit-serially. Each \STR \tile uses a \textit{Reducer} unit to store the output neurons in NM. 

The rest of this section is organized as follows: Section~\ref{sec:approach} discusses the approach \STR uses to enable bit-serial processing of neurons while matching or exceeding \BASE's performance. Section~\ref{sec:tile} describes the organization and operation of \STR's tiles. Section~\ref{sec:computeunit} describes the core bit-serial inner-product units used in the tiles.  Section~\ref{sec:inputneurons} describes the Dispatcher, and Section~\ref{sec:outputneurons} descibes the Reducers.  Section~\ref{sec:fclayer} describes how \STR implements the non-convolutional layers, and Section~\ref{sec:metadata} concludes the description of \STR by explaining how the per layer precision information is communicated. Finally, Sections~\ref{sec:replication} and~Section~\ref{sec:decompose} 
compare \STR's approach with increasing the number of \tiles and with using decomposable units respectively.

\subsection{Processing Approach}
\label{sec:approach}
Since \STR uses bit-serial computation for neurons, it needs to process more neurons in parallel than \BASE to maintain performance when the maximum precision is used. Specifically, in the worst case, \STR needs 16 cycles to calculate a product involving a 16-bit neuron. Given that a \BASE \tile processes a 16 neuron brick in parallel, \STR needs to process 16 bricks, or 256 neurons in parallel. The parallelism of convolutional layers offers a multitude of options for processing neurons in parallel. \STR opts to process 16 windows in parallel using a neuron brick from each window so that the same 16 synapses from each of the 16 filters can be used to calculate $16\times 16$ output neurons in parallel. For example, for a layer with a stride of 2 an \STR \tile will processes 16 neuron bricks $n_B(x,y,i)$, $n_B(x+2,y,i)$ through $n_B(x+31,y,i)$
in parallel, a single bit per neuron per cycle.  
In this case, assuming that the \tile processes filters $f_{i}$ though $f_{i+15}$, after $p$ cycles it would produce the following \textit{partial} output neurons:
$o_B(x/2,y/2,f_{i})$, through $o_B(x/2+15,y,f_{i})$, 
or a \textit{pallet} of 16 contiguous on the $x$ dimension output neuron bricks. Whereas \BASE would process 16 neuron bricks over 16 cycles, \STR processes them concurrently but bit-serially over $p$ cycles. If $p$ is less than 16, \STR will outperform \BASE by $16/p$, and when $p$ is 16, \STR will match \BASE's performance. 



\subsection{Tile Organization and Operation}
\label{sec:tile}
 As Figure~\ref{fig:stripes-overview} shows the \tile is organized as follows: the \tile's NBin is logically organized in 16 \textit{window lanes}, each a group of 16 bit-serial neuron lanes for a total of 256 neuron lanes. Each window lane processes one of the 16 input neuron array windows. The SB is identical to \BASE and is logically organized in 16 filter lanes, each containing 16 synapse lanes.
The SB and NBin connect to an array of $16\times 16$ \textit{Serial Inner Product} (SIP) subunits, where each SIP is responsible for one output neuron. The SIP($f$,$w$) at row $f$ and column $w$ processes filter lane $f$ and neuron window $w$. The SB filter lane $f$ connects via a bus to all SIPs along row $f$, whereas the NBin window lane $w$ connects via a bus to all SIPs along column $w$.
Each SIP accepts as input 16 neuron bits and a synapse brick which is latched onto a \textit{synapse register} (SR). The SR is needed to support fully connected layers as Section \ref{sec:fclayer} explains.
 The figure shows simplified SIPs and a more complete description is given in Section \ref{sec:computeunit}. Each SIP contains a 16-input adder tree for a total of 256 16-input adder trees whereas \BASE requires only 16 one per IP. It may seem that would increase area considerably for \STR, however, each \BASE IP requires 256 2-input 16-bit multipliers, whereas \STR requires none. Section~\ref{sec:evaluation} will show that the \STR's NFU area overhead is \NFUareaoverhead compared to \BASE.


Processing in a \tile proceeds in phases of $p$ cycles cycles each, where $p$ is the precision of neurons in bits.  At the first cycle of a phase, SB provides 16 bricks of 16-bit synapses, one brick per filter. Each SIP latches its corresponding synapse brick in its SR. Every cycle, NBin provides 256 neuron bits and 
%While in \BASE each synapse is multiplied with only one neuron, in \STR each synapse is broadcast over all SIPs along the corresponding row and in total is ANDed with 16 neurons, one from each window. 
each neuron bit is bit-wise \textit{ANDed} with 16 synapses, one per SIP along the same column. Each AND operation produces a 16-bit \textit{term}. Thus, each SIP calculates 16 terms corresponding to one filter and one window. The SIP sums its 16 terms into a partial output neuron using a dedicated 16-input adder tree. For the remaining $p-1$ cycles of a phase, each SIP shifts its partial output neurons by one bit, while accumulating another 16 terms implementing bit-serial multiplication. After $p$ cycles, an output neuron pallet, that is 256 16-bit partial output neurons are produced in full.  


\begin{figure}[!t]
\centering
\includegraphics[scale=0.5]{figures/systems-overview}
\caption{
Overview of the system components and their communication. a) \BASE. b) \STRL.
}
\label{fig:systems-overview}
\end{figure}



\subsection{SIP: Bit-Serial Inner-Product Units}
\label{sec:computeunit}
In the described implementation, \STR \nfus produce 256 output neurons concurrently and bit-serially over multiple cycles. Each output neuron computation is an inner product. Whereas the baseline design calculates this inner product 16 input neurons and 16 synapses at a time, \STR does so differently. For each output neuron and at each cycle, 1 bit from each of 16 input neurons along with 16 synapses are combined. 

Multiplying neurons bit-serially is straightforward where the neuron is fed serially and the synapse is fed in-parallel. Spefically, given an input neuron $n$ of length $p$ bits, $n$'s binary representation is \(\sum_{b=0}^{p}{n_b \times 2^b }\), where \(n_b\) is $n$'s b\(^{th}\) bit. 
Given a synapse $s$, the multiplication $s \times n$ can be rewritten as \(\sum_{b=0}^{p}{2^b \times n_b \times s  }\). This leads to a circuit implementation where $n_b \times s$ is an AND, multiplication with $2^b$ is a shift and the summation is performed with an accumulator over $p$ cycles. 

To apply this naively to \BASE, we could simply convert each of the parallel multipliers to serial ones. 
However, we can simplify this design using the commutative property of addition as described by White \cite{white_applications_1989}.
Formally, the terms of the inner product of Equation~\ref{eq:convolution} can be reorganized as follows where $n^b$ the b\textit{th} bit of $n$ and $Ni=16$ is the size of the vectors. 

\begin{gather*}
\small
\begin{split}
\sum_{i=0}^{N_i-1}{s_i\times n_i} = \sum_{i=0}^{N_i-1}{s_i\times \sum_{b=0}^{p-1}{n_i^b \times 2^b }} = 
\sum_{b=0}^{p-1}{2^b \times \sum_{i=0}^{N_i-1}{n_i^b \times s_i}}
\end{split}
\end{gather*}


\begin{figure}[]
\centering
\includegraphics[scale=0.6]{figures/SIP-internals}
\caption{SIP components.}
%\PJ{mux the max out and o_nbout, specify \<\<1} }
\label{fig:SIP-internals}
\end{figure}

In terms of logic, this shows that we can first perform the reduction on the products $n^b_i \times s_i$ with an adder tree, and then perform the shift and accumulate on the resulting sum. 
This simplifies the serial inner product unit by moving the shifted accumulator from each of the 16 inputs in the adder tree to just one on the output. 
Figure~\ref{fig:SIP-internals} shows the resulting serial inner product circuit. 
To support signed 2's complement neurons, the SIP must subtract the synapse corresponding to the MSB from the partial sum when MSB is 1. 
This is done with negation blocks for each synpase before the adder tree.  
To support inner products larger than $Ni$ data is read back from NBout and used to initialize the accumulator. 
Each SIP also includes a comparator (max) to support max pooling layers.  



\subsection{Dispatcher: Supplying Input Neurons} 
\label{sec:inputneurons}
\BASE's neuron memory broadcasts a brick, that is 16 16-bit neurons, or 256 bits per cycle to all \tiles and each \tile processes the same brick over different filters. \STR needs to also broadcast 256 bits per cycle to all \tiles but where each bit corresponds to a different neuron. \STR currently opts to maintain the same neuron storage container format in central neuron memory (NM) as in \BASE aligning each neuron at a 16-bit granularity. A \textit{Dispatcher} unit is tasked with reading neurons from NM and feeding them to the \STR \tiles bit-serially.  Section~\ref{sec:neuronmap} describes how neurons are read from the NM, and Section~\ref{sec:dispatcher} describes how the Dispatcher combines the raw neuron data from the NM and feeds them serially to the \tiles.

\begin{figure}[]
\centering
\includegraphics[scale=0.55]{figures/dispatcher}
\caption{Dispatcher.
}
\label{fig:dispatcher}
\end{figure}

\subsubsection{Reading the Neurons from NM} 
\label{sec:neuronmap}
Reading the necessary neurons from NM is best understood by first considering a layer using a unit stride. In this case, at each cycle, the \STR \nfus need to be fed with bits from 16 contiguous along the $x$ dimension bricks: 
$n_B(x,y,i))$, $n_B(x+1,y,i)$ through $n_B(x+15,y,i)$. 
%$n(x,y,i)...n(x,y,i+15)$, $n(x+1,y,i)...n(x+1,y,i+15)$ through $n(x+15,y,i)...n(x+15,y,i+15)$. 
Provided that these 16 neuron slices can be read in parallel, all the dispatcher has to do, is feed them bit serially over the next $p$ cycles. To enable reading the 16 bricks in parallel \STR maps them on consecutive locations in NM. In many cases, this will result in the 16 bricks being stored onto the same NM row. In this case, the dispatcher can read them all in a single cycle (given that the 2MB NM comprises several subarrays, reading 256 neurons in parallel is feasible).

Depending on the input neuron array $y$ dimension, the 16 bricks may spread over two NM rows 
%as the example of Figure~\ref{fig:crossbar-example} shows 
(this is similar to reading a misaligned block from a data cache). In this case, the dispatcher will have to read and combine the appropriate bricks from up to two rows over two cycles before it can feed the \STR \tiles. As long as $p$ is at least 2, the next set of 16 bricks will not be needed until $p$ cycles have elapsed. Accordingly, the whole process can be pipelined and thus the \STR \nfus can be kept busy all the time.

% \begin{figure}[]
% \centering
% \includegraphics[scale=0.55]{figures/shuffling-stride1}
% \caption{Shuffler example when the input bricks do not all fall into the same NM row and the stride is 1.}
% \label{fig:crossbar-example}
% \end{figure}

Figure~\ref{fig:memory-mapping} shows an example with two windows and stride of 2. When the stride $S$ is more than one, the 16 bricks could be spread over $R=min[S+1, 16]$ rows. Accordingly, the dispatcher will have to read $R$ rows over $R$ cycles before feeding the next set of 256 neurons to the \tiles. As long as $R$ is less then $p$ there will be enough time to keep the \nfus busy all the time. Only when $R$ is more than $p$ the \nfus will have to stall and for $R-p$ cycles. It may be possible to reduce the number of rows that the dispatcher needs to read by mapping bricks to NM taking into account the stride. However, as Section~\ref{sec:evaluation} will show, such stalls were observed only for one layer of LeNet and only for 2\% of the time. Accordingly, this is left for future work. 


\begin{figure}[tbp]
\centering
\includegraphics[scale=0.5]{figures/memory-mapping}
\caption{Memory mapping of elements from different windows.
}
\label{fig:memory-mapping}
\end{figure}


\subsubsection{Dispatcher Design}
\label{sec:dispatcher}
As the previous section described, given a layer stride $S$, the dispatcher needs to read up to $max[S+1,16]$ rows, one per cycle to collect 16 bricks. Given these 16 bricks, the dispatcher then needs to send one bit from each of the 256 neurons they contain, for a total 256 bits per cycle, over $p$ cycles to the \STR \tiles.

As Figure~\ref{fig:dispatcher} shows, the dispatcher is composed of two parts: a  \textit{Shuffler} and a \textit{Transposer}. The Shuffler reads 16 bricks from NM and the Transposer communicates them bit-serially to the \tiles. The dispatcher needs to communicate a new set of 16 bricks every $p$ cycles.

\noindent\textbf{Shuffler:} The Suffler's goal is to collect the 16 bricks that are needed to keep the \STR \nfus busy over $p$ cycles. The collection of the next group of 16 bricks, can be overlapped with the processing of the current group, hence the Shuffler needs to collect a 16 brick group every $p$ cycles.

Each cycle, the Shuffler reads a row of 256 neurons from NM. Given that bricks are stored contiguously in NM every row contains 16 bricks, however, these many not all be the bricks currently needed. 
A 16-to-1 multiplexer per output brick is sufficient to select the appropriate brick when that appears on the input row. Accordingly, the Shuffler comprises 16 16-to-1 256-bit (one brick of 16 neuron 16-bit containers) multiplexers. The input neurons are collected on 256 16-bit registers organized in groups of 16, one per input brick. Once the Shuffler has collected all 16 bricks, it transfers them to the input registers of the Transposer. 

\noindent\textbf{Transposer:} 
The Transposer converts the neurons read from memory by the Shuffler to serial bit streams. Once the shuffler has collected all 16 bricks, it writes them bit-parallel into 256 16-bit registers. Each register provides a 16-bit bit-parallel write port, and a single-bit bit-serial read port. Over the next $p$ cycles, the Transposer outputs one bit per neuron for a total of 256 bits per cycle. These are broadcast to all NFUs using the same interconnect as in \BASE. 




 

\subsection{Reducers: Writing the Output Neurons}
\label{sec:outputneurons}
\STR's NFUs produce output neurons in \BASE's 16-bit fixed-point format. The \textit{Reducer} units serve a dual purpose: 1)~convert to the precision needed by the output layer, and 2)~write the output neuron bricks to NM.


Writing the output neurons back to NM uses the same interconnect as in \BASE. The only difference is that since \STR outperforms \BASE, it exhibits higher output neuron bandwidth demand. Fortunately, since calculating an output neuron requires processing a full input neuron window, there is enough time to meet this demand with the exiting interconnect. 
Specifically, while \BASE produces a single output neuron brick, or 16 output neurons concurrently (e.g., 
$o_B(x,y,f_{i})$), 
%$o(x,y,f_{i})...o(x,y,f_{i+15})$), 
\STR produces a pallet or 256 output neurons comprising 16 contiguous along the $x$ dimension bricks, (e.g.,  $o_B(x,y,f_{i}))$ through $o_B(x+15,y,f_{i})$).
%$o(x,y,f_{i})...o(x,y,f_{i+15})$ through $o(x+15,y,f_{i})...o(x+15,y,f_{i+15})$).
This pallet needs to be stored contiguously in the NM address space as expected by the Dispatcher when processing the next layer. \STR's \tiles send a single brick at a time as in the baseline and take multiple cycles to write all 16. Since the \tiles write a single brick per cycle, and since bricks never span an NM row, there is no need for supporting misaligned brick writes.

Since \STR outperforms \BASE its computational throughput is increased by $16/p$. If a layer is relatively small, it is in principle possible to need extra cycles to drain all output neurons. However, even in the baseline output neurons typically take hundreds of cycles to be computed as producing an output neuron requires processing a full input neuron window. Accordingly, there is sufficient time to write all output bricks. No stalls were ever observed for any of the networks studied.

% \begin{figure}[]
% \centering
% \includegraphics[scale=0.5]{figures/round}
% \caption{Encoder modifies output neurons before being written.\fixme{what are the inputs? What is instead each box?} }
% \label{fig:round}
% \end{figure}




\subsection{Executing Other Layers}
\label{sec:fclayer}
%one large matrix-vector multiplication, with a vector of neurons and a matrix of synapses (the filter size matches that of the input neuron array).
%The underlying inner product computations are performed like those in convolution layers. 
%However, in this case synapses are only used once, so the strategy of broadcasting each synapse to multiple neurons doesn't work. 
%Fully connected layers can be thought of as convolutions with only one window, one which covers the entire set of input neurons. 
%As such, we are unable to exploit multi-window parallelism to broadcast weights to each window. 
%The underlying inner product computations are performed like those in convolution layers. 
%However, in this case synapses are only used once, so the strategy of broadcasting each synapse to multiple neurons doesn't work. 
%Fully connected layers can be thought of as convolutions with only one window, one which covers the entire set of input neurons. 
%As such, we are unable to exploit multi-window parallelism to broadcast weights to each window. 


\noindent\textbf{Fully Connected:} 
\BASE computes fully connected (FC) layers as a convolution layer where the filter dimensions match that of the input neuron array.
In this case there is only one window necessitating a different data access and execution schedule to match \BASE's performance. 
When processing a convolutional layer, the synapses are read ony once every $p$ cycles. To process an FC layer, the \nfu can load synapses in a round-robin fashion one SIP column per cycle via the single SB read port and bus, keeping all SIPs busy processing neurons. 
%held at the input of each SIP and reused over $p$ cycles while the serial neuron bits are fed in. 
%As such, there is additional SB bandwidth to load synapses in a round-robin fashion one SIP column per cycle via the single SB read port and bus, keeping all SIPs busy processing neurons. 
For example, with reference to Figure \ref{fig:stripes-overview}, a \nfu can load 256 synapses to SIP(0,0)..SIP(0,15) in cycle 0, then load the next 256 synapses to SIP(1,0)..SIP(1,15) in cycle 1, etc. The loading of synapses can be overlapped with processing neurons by staggering the neuron stream to synchronize with the loading of synapses. This mode of operation (Round robin synapse loading and staggered neurons streams) only requires modification to the control.
Table~\ref{tab:fc} shows an example, illustrating how synapse loading and computation is overlapped.
\begin{table}[t]
\small
\centering
\begin{tabular}{|l|}
\hline
\textbf{Cycle 0:} \\
\enspace \textbf{SIP(0,0)...SIP(0,15):} \textbf{latch} $s_B^{0}(0,0,0),...,s^{15}_B(0,0,0)$ \\
\enspace\enspace via window lane 0: receive bit 0 of  $n_B(0,0,0)$ \\
\hline
\textbf{Cycle 1:}  \\
\enspace \textbf{SIP(0,0)...SIP(0,15):}\\
\enspace\enspace via window lane 0: receive bit 1 of  $n_B(0,0,0)$\\
\enspace \textbf{SIP(1,0)...SIP(1,15):} \textbf{latch}  $s^{0}_B(1,0,0),...,s^{15}_B(1,0,0)$ \\
\enspace\enspace via window lane 1: receive bit 0 of  $n_B(1,0,0)$ \\
\hline
...\\
\hline
\textbf{Cycle 15:} Fully Utilized\\
\enspace \textbf{SIP(0,0)...SIP(0,15):} \\
\enspace\enspace  via window lane 0: receive bit 15 of  $n_B(0,0,0)$ \\
\enspace \textbf{SIP(1,0)...SIP(1,15):}\\
\enspace\enspace  via window lane 1: receive bit 14 of  $n_B(1,0,0)$\\
\enspace...\\
\enspace \textbf{SIP(15,0)...SIP(15,15):} \textbf{latch}  $s^{0}_B(15,0,0),...,s^{15}_B(15,0,0)$ \\
\enspace\enspace  via window lane 15: receive bit 0 of  $n_B(15,0,0)$\\\hline
\textbf{Cycle 16:} Fully Utilized\\
\enspace \textbf{SIP(0,0)...SIP(0,15):} \textbf{latch} $s^{0}_B(0,0,16),...,s^{15}_B(0,0,16)$ \\
\enspace\enspace  via window lane 0: receive bit 0 of  $n_B(0,0,16)$ \\
\enspace...\\
\enspace \textbf{SIP(15,0)...SIP(15,15):}\\
\enspace\enspace  via window lane 15: receive bit 1 of  $n_B(15,0,0)$\\\hline
\end{tabular}
\caption{Processing an FC layer: The first 17 cycles.}
\label{tab:fc}
\end{table}
This approach improves performance for FC layers when \textit{batching} is used, a common strategy when synapse bandwidth becomes a bottleneck. 
Batching computes each layer over multiple images at a time, so that synapses can be reused for neurons from different images. In this case, each synapse loaded to an SIP would be used for $p \times b$ cycles, where $b$ is the batch size. 
While there is no performance improvement over \BASE when processing a single image, using a shorter precision in FC layers reduces energy by avoiding computations on each SIP column for $16-p$ cycles of every $16$ cycles.
There is a small overhead from staggering the neuron streams, which is 0.16\% of the layer runtime on average. The potential for further improving performance by accelerating FC layers is very small since they account for a small fraction of the overall execution time. Furthermore, the current trend in DNNs is for reducing or eliminating the number of FC layers, e.g., \cite{he_deep_2015-1}.



\noindent\textbf{Other Layers: }Local response normalization and average pooling layers use the serial multipliers analogously to how the multipliers are used in \BASE.
Max pooling layers are supported with comparators in the SIPs. 
For all these layers data is still read in serially to increase the effective bandwidth of the interconnect, which can provide 256 words over $p$ cycles. 
As such they will all experience speedup inversely to the precision of the data. 

\subsection{Communicating the Per Layer Precisions}
\label{sec:metadata}
This work assumes that the per layer precisions are pre-calculated using a method such as that described in Section~\ref{sec:methodology} and provided along with the network's other metadata such as the dimensions, padding and stride of each layer. Several complete profiles of per layer precisions can be supplied by the DNN to enable accuracy vs. performance trade offs at run-time. This metadata information is read by the \STR controller and used to control the operation of the \nfus, the Dispatcher and the Reducers.

\subsection{STR vs. More Bit-Parallel Tiles}
\label{sec:replication}

Since the convolutional layers are highly parallel, improving \BASE's performance is possible by exploiting parallelism by adding more tiles. As Section~\ref{sec:evaluation} shows, \STR increases \tile area by \tileareaoverhead. Assuming ideal performance scaling, we could instead use this extra area to introduce an additional \tileareaoverhead more \tiles. In reality, ideal scaling will not be possible as it may not be possible to keep all neuron lanes busy. For example, a \BASE chip can be fully utilized only as long as there are multiple of 256 filters in a layer (16 filters in each of the 16 \tiles). As a result, depending on the layer, there are cases where \nfus are underutilized and having more \nfus will make such cases more common.

Even under the unrealistic assumption that \BASE's performance can be scaled by \tileareaoverhead with the same area overhead and \STR, Section~\ref{sec:evaluation} shows that \STR outperforms this alternative and thus offers a better area vs. performance scaling. Furthermore, \STR's approach enables static or run-time performance vs. accuracy trade offs which are not possible with the baseline design.


\subsection{STR vs. Decomposable Processing Units}
\label{sec:decompose}
A common approach to gaining performance from reduced precision is to use decomposable multipliers and adders~\cite{mmx}
\cite{tan_multiple-precision_2003-1}
\cite{huang_low-cost_2012}.
For example, a 16-bit adder can easily be configured as two 8-bit adders with minimal overhead. This approach is commonly used in multimedia instruction set extensions of general purpose processors, e.g.,~\cite{mmx}. Since this does not increase latency of each operation it is simple to increase computational throughput. 

When considering the characteristics of neural networks~\cite{judd:reduced}, decomposable units have three constraints that disadvantage them: 
1)~Decomposable units are typically constrained to power-of-2 precisions, meaning they cannot yield all of the potential benefit of variable reduced precision. For example, a layer requiring only 9 bits would still need to use 16.
2)~Decomposable units require both inputs to be the same width.  In the case of neural networks these are the weights and the neurons, weights typically require more than 8 bits~\cite{judd:reduced} and as a result many layers will not see improvement. 3)~Finally, if the baseline multipliers and adder trees were decomposable, the largest precision of the data and weights would have to be chosen for each layer.

Section~\ref{sec:eval:decomposable} demonstrates that \STR outperforms an idealized decomposable unit based \BASE design.  

% \subsubsection{Single vs. Multiple Windows}
% \fixme{if we end up needing space, we can remove these two sections}Since \STR as described processes neurons bit-serially, it uses cross neuron parallelism to maintain throughput on par with the baseline design when the full precision is needed. In our description thus far this parallelism was found by processing in parallel multiple output neurons (windows). The advantage of this approach is that the same set of synapses can be reused, thus keeping the SB design the same as in the baseline. Other approaches are possible. For example, we could have instead processed additional neurons from the same window along the $i$ dimension. The advantage here would be that all partial products would feed into the same output neuron, a property that may lead to additional circuit level optimizations in the adder trees but would require reading $16\times$ as many synapses. This is left for future work.
% %Furthermore, this approach would enable skipping of all inneffectual neurons using the design of Albericio et al. \fixme{[ISCA]} \JA{this would say it's us}.\PJ{lets not mention this point} However, this approach requires $16\times$ as many synapses to be provided, for a total of $4K$ synapses. Accordingly, a study of this approach is left for future work.
% \subsubsection{Packing of Neurons in Memory}
% \STR currently uses 16-bit containers for neurons in NM. However, it may be possible to reduce NM bandwidth requirements if neurons are instead stored natively using only as many bits as necessary. Futhermore, it may be possible to reduce NM footprint even further by using the techniques of Deep Compression~\cite{han_deep_2015-1}. However, either approach will affect the Dispatcher and Reducer designs may require more complicated shuffling networks. Accordingly, this is left for future work.

% %Could we pack the neurons in memory similar to Proteus of the Stanford work? Say that this is an option and future work?
% %\subsubsection{Neurons vs. Synapses}
% %\STR processes neurons bit-serially. 
% %To process synapses bit-serially, and maintain the compute bandwidth of the baseline, would require 16x the neurons. The units themselves would not chance, but the neurons are broadcast across the chip using a fat tree, and the physical bandwidth would need to be increased upto 16x to support precisions down to 1 bit.    





